A Survey on 5G Radio Access Network Energy Efficiency: Massive MIMO, Lean Carrier Design, Sleep Modes, and Machine Learning

Cellular networks have changed the world we are living in, and the fifth generation (5G) of radio technology is expected to further revolutionise our everyday lives, by enabling a high degree of automation, through its larger capacity, massive connectivity, and ultra-reliable low-latency communications. In addition, the third generation partnership project (3GPP) new radio (NR) specification also provides tools to significantly decrease the energy consumption and the green house emissions of next generations networks, thus contributing towards information and communication technology (ICT) sustainability targets. In this survey paper, we thoroughly review the state-of-the-art on current energy efficiency research. We first categorise and carefully analyse the different power consumption models and energy efficiency metrics, which have helped to make progress on the understanding of green networks. Then, as a main contribution, we survey in detail -- from a theoretical and a practical viewpoint -- the main energy efficiency enabling technologies that 3GPP NR provides, together with their main benefits and challenges. Special attention is paid to four key enabling technologies, i.e., massive multiple-input multiple-output (MIMO), lean carrier design, and advanced idle modes, together with the role of artificial intelligence capabilities. We dive into their implementation and operational details, and thoroughly discuss their optimal operation points and theoretical-trade-offs from an energy consumption perspective. This will help the reader to grasp the fundamentals of -- and the status on -- green networking. Finally, the areas of research where more effort is needed to make future networks greener are also discussed.

==> sections/Outline.tex <==
\section{Introduction} \textcolor{blue}{David}
\label{sec:intro}

\begin{itemize}
\item{The 5G communications era }
    \begin{itemize}
    \item	Users and enterprises demand more of everything, e.g. capacity, latency, reliability, etc.
    \item 5G developed to meet such user and enterprise requirements
        \begin{itemize}
        \item This is the place to touch upon the main 5G features, and how they relate to capacity, latency, reliability, etc.
        \end{itemize}
    \end{itemize}
\item{5G network power consumption-related concerns}
    \begin{itemize}
    \item{5G can meet the above requirements, but there are social and energy related concerns about the operation of this new type of network}
        \begin{itemize}
        \item People is worried about 5G eco-friendliness and others (e.g. health)
        \item MNOs are also worried about the above plus energy bills
        \end{itemize}
    \end{itemize}
\item 5G as an energy efficiency enabler
    \begin{itemize}
    \item {Position 5G, in general, as a more energy efficient technology than any other preceding one using recent reports and surveys. However, acknowledge the need to decrease power consumption.}
    \item {Describe the 5G key features that can allow such power consumption reductions in more detail}
        \begin{itemize}
        \item {	Lean carrier}
        \item {	Massive MIMO} 
        \item {	Advanced idle mode support}
        \item {	ML}
        \end{itemize}
    \end{itemize}
\item{Need for intelligent 5G networks}          
    \begin{itemize}
    \item {Given the above 5G potential for power consumption reduction, highlight the need for intelligent optimization techniques that help us to realize those saving. Here we can refer to the effort done by, e.g. the 3GPP and the ETSI in this context}
    \item {Stress that these techniques will find the most gains when aware of UE distributions, traffic variability, mobility patterns and the current power consumption itself}
    \item{Stress the need to care for QoS guarantees for the users, and introduce the importance of understanding tradeoffs. We may trade capacity/delay/reliability for energy efficiency }
    \end{itemize}
\item{Comparison again other surveys}
    \begin{itemize}
    \item Clarify that we do not only focus on PHY layer techniques as other surveys and that we have a more holistic approach. Motivate our choice
    \end{itemize}
\item{Structure of the paper}
\end{itemize}

\section{Power Consumption Models} \textcolor{blue}{Antonio}
\begin{itemize}
    \item {Classify and discuss energy consumption models }
\end{itemize}

\section{Energy Efficiency Metrics} \textcolor{blue}{Antonio}
\begin{itemize}
    \item {Classify and discuss energy efficiency metrics }
\end{itemize}

\section{M-MIMO} 
\begin{itemize}
\item \textcolor{blue}{ David}
Go in more detail on the key role of massive MIMO in 5G. Discuss the importance of massive MIMO to enhance capacity, but also how the more antennas consume more power, etc. 
\item 
Show a general numerical comparison between 5G vs LTE energy efficiency with massive MIMO at heart, showing how massive MIMO can improve EE and thus the more antennas (M. Debbah slides can help here)
\item
Survey in detail massive MIMO literature 
    \begin{itemize}
    \item {Single cell analysis } \textcolor{blue}{Nicola}
            \begin{itemize}
            \item {Discuss that the state of the art is quite complete, and that tradeoffs are well understood}
            \item {ii.	Go over all interesting papers and highlight the main findings, i.e. how EE changes with number of antennas, users, transmit power, etc. }
            \item{Provide table to summarize}
            \end{itemize}
    \item {Multi cell} \textcolor{blue}{ David}
            \begin{itemize}
            \item {Discuss that the state of the art is not as complete due to complexity, and that most papers do not focus on tradeoffs but on optimization problems}
            \item {Go over all interesting papers and highlight the main findings}
            \item{Provide table to summarize}
            \end{itemize}
    \end{itemize}
\end{itemize}

\section{ON/OFF} \textcolor{blue}{Antonio}
Once massive MIMO and is configuration is understood, explain the need and survey ON/OFF techniques taking into account different domains. Few papers in each category will suffice. I would put emphasis on how these techniques need information of UE distributions, traffic and mobility to best perform 
Include 3GPP NR sleeping time and duration
\begin{itemize}
\item {Time}
        \begin{itemize}
        \item {Here we focus on lean carrier and discontinuous transmissions optimization techniques}
        \end{itemize}
\item {Cell and carriers}
        \begin{itemize}
        \item {Here we focus on multicarrier networks and on carrier ON/OFF optimization techniques. BS ON/OFF optimization techniques (note that this last one is a particular case of carrier ON/OFF)}
        \end{itemize}
\item {Antenna domain}
        \begin{itemize}
        \item {Here we focus on antennas ON/OFF for massive MIMO case (there may be little literature here)}
        \end{itemize}
\item{Feel free to include other features that you believe relevant}
\end{itemize}

\section{Machine learning}
Discuss the challenges of understanding UE distributions, traffic and mobility, and how ML is a natural science that can help us to understand those and optimize the functioning of the about ON/OFF techniques. Here, I would pick an example, for instance base station or carrier ON/OFF optimization techniques, and discuss the following
\begin{itemize}
\item {Data}
        \begin{itemize}
        \item {Describe challenges in data gathering and survey existing work}
        \end{itemize}
\item {Prediction}
        \begin{itemize}
        \item {Describe challenges in prediction and survey existing work}
        \item \textcolor{red}{ADD: Besides load, what literature focuses on that is related to our problem? (energy consumption? QoS?)}
        \end{itemize}
\item {Algorithm}
        \begin{itemize}
        \item {Survey existing work on reinforcement and data-driven learning schemes and discuss their gains and challenges with respect to classical optimization}
        \end{itemize}
\item{Feel free to include other features that you believe relevant}
\end{itemize}

\section{New directions of research }
Here is our opportunity to show some of our work and share our views on how data can help theoretical understanding and the development of practical algorithms.
\begin{itemize}
\item RIS can be one enabler that we discuss here
\end{itemize}

\section{Conclusion}
\label{sec:conclusion}
